High-order interpolatory Serendipity Virtual Element Method for semilinear parabolic problems

We propose an efficient method for the numerical approximation of a general class of two dimensional semilinear parabolic problems on polygonal meshes. The proposed approach takes advantage of the properties of the serendipity version of the Virtual Element Method, which not only reduces the number of degrees of freedom compared to the original Virtual Element Method, but also allows the introduction of an approximation of the nonlinear term that is computable from the degrees of freedom of the discrete solution with a low computational cost, thus significantly improving the efficiency of the method. An error analysis for the semi-discrete formulation is carried out, and an optimal estimate for the error in the $L_2$-norm is obtained. The accuracy and efficiency of the proposed method when combined with a second order Strang operator splitting time discretization is illustrated in our numerical experiments, with approximations up to order $6$.

==> makefile <==
DOCUMENT = article
DVIPS_OPTS  = -Ppdf -G0 -tletter
PS2PDF_OPTS = -dSubsetFonts=true -dEmbedAllFonts=true
PDFLATEX_OPTS = -shell-escape

default : pdf
pdf:
	pdflatex  $(PDFLATEX_OPTS) $(DOCUMENT);\
	bibtex $(DOCUMENT);\
	pdflatex $(PDFLATEX_OPTS) $(DOCUMENT);\
	pdflatex $(PDFLATEX_OPTS) $(DOCUMENT);\
	make clean;
	
clean:
	/bin/rm -rf *.log *.ps *.toc *.dvi *.lof *.blg\
	 *.backup *.aux *.spl *.out

